Uniqueness and root-Lipschitz regularity for a degenerate heat equation

We consider nonnegative solutions of the quasilinear heat equation $\partial_t u = \tfrac{1}{2} u \partial_x^2 u$ in one dimension. Our solutions may vanish and may be unbounded. The equation is then degenerate, and weak solutions are generally nonunique. We introduce a notion of strong solution that ensures uniqueness. For suitable initial data, we prove a lower bound on the time for which a strong solution $u$ exists and $\sqrt{u}$ remains globally Lipschitz in space. In a companion paper, we show that this condition is important in the study of two-dimensional nonlinear stochastic heat equations.

==> NLH-macros.tex <==
\newcommand*{\R}{\mathbb{R}}
\providecommand*{\C}{}
\renewcommand*{\C}{\mathbb{C}}
\newcommand*{\N}{\mathbb{N}}
\newcommand*{\Z}{\mathbb{Z}}
\newcommand*{\Q}{\mathbb{Q}}
\newcommand*{\T}{\mathbb{T}}
\newcommand*{\A}{\mathbb{A}}
\newcommand*{\E}{\mathbb{E}}
\newcommand*{\K}{\mathbb{K}}
\newcommand*{\F}{\mathbb{F}}
\newcommand*{\D}{\mathbb{D}}
\newcommand*{\Ham}{\mathbb{H}}
\newcommand*{\hs}{\mathbb{H}}
\newcommand*{\cc}{\mathrm{c}}
\newcommand*{\loc}{\mathrm{loc}}
\renewcommand*{\P}{\mathbb{P}}
\newcommand*{\e}{\mathrm{e}}
\newcommand*{\eps}{\varepsilon}
\newcommand*{\al}{\alpha}
\newcommand*{\Om}{\Omega}
\newcommand*{\bd}{\partial}
\newcommand*{\h}[1]{\hat{#1}}
\newcommand*{\s}[1]{\mathscr{#1}}
\newcommand*{\m}[1]{\mathcal{#1}}
\newcommand*{\f}[1]{\mathfrak{#1}}
\newcommand*{\dn}{\mathrm{d}}
\newcommand*{\diff}{\mathrm{d}}
\newcommand*{\ds}{\,\mathrm{d}}
\renewcommand*{\d}{\;\mathrm{d}}
\newcommand*{\Der}{\mathrm{D}}
\newcommand*{\der}[2]{\frac{\dn #1}{\dn #2}}
\newcommand*{\pa}[2]{\frac{\partial #1}{\partial #2}}
\newcommand*{\abs}[1]{\left |#1 \right|}
\newcommand*{\abss}[1]{|#1|}
\newcommand*{\absb}[1]{\big|#1\big|}
\newcommand*{\norm}[1]{\left \|#1 \right\|}
\newcommand*{\norms}[1]{\|#1\|}
\newcommand*{\normb}[1]{\big\|#1 \big\|}
\newcommand*{\op}[1]{\operatorname{#1}}
\newcommand*{\sgn}{\op{sgn}}
\newcommand*{\ti}[1]{\tilde{#1}}
\newcommand*{\ubar}[1]{\underline{#1}}
\newcommand*{\tbf}[1]{\textup{\textbf{#1}}}
\newcommand*{\trm}[1]{\textup{\textrm{#1}}}
\newcommand*{\id}[1]{\op{id}_{#1}}
\newcommand*{\anon}{\,\cdot\,}
\renewcommand*{\Re}{\op{Re}}
\renewcommand*{\Im}{\op{Im}}
\newcommand*{\Ker}{\op{ker}}
\newcommand*{\Image}{\op{im}}
\newcommand*{\Span}{\op{span}}
\newcommand*{\supp}{\op{supp}}
\newcommand*{\trans}[1]{\tensor*[^t]{#1}{}}
\newcommand*{\smooth}[1]{\m{C}_c^\infty(#1)}
\newcommand*{\arccot}{\op{arccot}}
\newcommand*{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand*{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand*{\noorm}[1]{\left|\left \|#1 \right\|\right|}
\newcommand*{\MLoc}{\m M_{c,\text{loc}}}
\newcommand*{\BM}{Brownian motion~}
\renewcommand*{\And}{\quad \text{and} \quad}
\newcommand*{\For}{\quad \text{for }}
\newcommand*{\ForAll}{\quad \text{for all }}
\newcommand*{\nab}{\nabla}
\newcommand*{\trdeg}{\op{tr\,deg}}
\newcommand*{\gr}{\op{gr}}
\newcommand*{\rees}{\op{Rees}}
\newcommand*{\Spec}{\op{Spec}}
\renewcommand*{\hom}[2]{\op{Hom}(#1, #2)}
\renewcommand*{\div}{\op{div}}
\newcommand*{\bbraket}[1]{\left \langle \! \left \langle #1 \right \rangle \! \right \rangle}
\newcommand*{\power}[1]{{#1}[\![X]\!]}
\newcommand*{\laurent}[1]{{#1}(\!(X)\!)}
\DeclareMathOperator*{\Dlim}{D-lim}
\DeclareMathOperator*{\Clim}{C-lim}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argsup}{arg\,sup}
\DeclareMathOperator*{\arginf}{arg\,inf}
\DeclareMathOperator*{\esssup}{ess\,sup}
\newcommand*{\mr}{\mathring}
\newcommand*{\smallO}{
  \mathchoice
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}%
    {\scalebox{.9}{$\scriptstyle\mathcal{O}$}}%
    {\scalebox{.9}{$\scriptscriptstyle\mathcal{O}$}}%
    {\scalebox{.6}{$\scriptscriptstyle\mathcal{O}$}}%
  }

\newcommand*{\iu}{\mathrm{i}}

\newcommand*{\smallbar}[1]{\overline{#1}}
\let\temp\bar
\let\bar\smallbar
\let\smallbar\temp
\let\temp\undefined

\newcommand{\CG}[1]{{\color{green!60!black}\textbf{CG:} #1}}
\newcommand{\AD}[1]{{\color{magenta}\textbf{AD:} #1}}
\newcommand{\ad}[1]{{\color{magenta}{#1}}}

